Maximal Extractable Value (MEV) Protection on a DAG

Many cryptocurrency platforms are vulnerable to Maximal Extractable Value (MEV) attacks, where a malicious consensus leader can inject transactions or change the order of user transactions to maximize its profit. A promising line of research in MEV mitigation is to enhance the Byzantine fault tolerance (BFT) consensus core of blockchains by new functionalities, like hiding transaction contents, such that malicious parties cannot analyze and exploit them until they are ordered. An orthogonal line of research demonstrates excellent performance for BFT protocols designed around Directed Acyclic Graphs (DAG). They provide high throughput by keeping high network utilization, decoupling transactions' dissemination from their metadata ordering, and encoding consensus logic efficiently over a DAG representing a causal ordering of disseminated messages. This paper explains how to combine these two advances. It introduces a DAG-based protocol called Fino, that integrates MEV-resistance features into DAG-based BFT without delaying the steady spreading of transactions by the DAG transport and with zero message overhead. The scheme operates without complex secret share verifiability or recoverability, and avoids costly threshold encryption.

==> sec/overview.tex <==
% -----*-------*---------*--------*---------------
\subsection{\BFT on a DAG}
The starting point for incorporating MEV protection 
is a \BFT protocol for the partial synchrony model, riding on a DAG transport.

There are many known \BFT solutions for partial synchrony, 
and more specifically, 
several recent solutions that ride on a DAG~\cite{danezis2022narwhal,giridharan2022bullshark,keidar2022cordial}.
When constructing Fino, we wanted to build MEV protection into a simple DAG-based \BFT solution, described below.
Notwithstanding, we remark that Fino's MEV protection can possibly be incorporated into other DAG-riding \BFT solutions.

We borrowed a subprotocol from Bullshark~\cite{giridharan2022bullshark} that deals with partial synchrony,
modifying it so that DAG transmissions would never stall waiting for \BFT protocol steps or timers.
Fino is different from the borrowed Bullshark component in that \BFT protocol 
steps (e.g., view changes, proposals, votes, and complaints) are injected into the DAG at any time, independent of DAG layers.
It uses \fino{broadcast()} (defined in \autoref{sec:pre}) to present these steps as payloads to the DAG transport, completely asynchronously,
while normal DAG transmissions continue.
A hallmark of the DAG-riding approach, which Fino preserves while adding Blind Order-Fairness, is zero message overhead.

In a nutshell, Fino's baseline \BFT solution works as follows:
\begin{itemize}

\item The protocol operates in a view-by-view manner.
Each view is numbered, as in \fino{view(r)}, and has a designated leader known to everyone.
Each view consists of {\em proposals}, {\em votes}, and {\em complaints} embedded inside the DAG
\item When a leader enters \fino{view(r)} it broadcasts \fino{proposal(r)}.
\item Other parties in \fino{view(r)}, after delivering \fino{proposal(r)}, 
broadcast \fino{vote(r)} that would causally follow \fino{proposal(r)}.
\item To indicate that \fino{view(r)} is not progressing,
parties broadcast \fino{complaint(r)}. 
Note that to guarantee progress during steady state, complaints are emitted only after allowing a leader sufficient time to broadcast and for votes to arrive.
\item A commit happens at \fino{view(r)} if there are F+1 votes for the leader proposal,
\item \fino{view(r+1)} is enabled either by a commit or by 2F+1 complaints.

\end{itemize}

A more detailed description is provided with MEV protection built into it, in \autoref{sec:fino}.

% --------* ---------- * ---------- * ----------- * ------------
\subsection{Incorporating ``\OTR'' on a DAG}

To order transactions blindly,
users choose for each transaction \fino{tx} a symmetric key \fino{tx-key},
and send \fino{tx} encrypted with it to \BFT parties.
The goal is to share \fino{tx-key} with parties,
such that a threshold greater than F and no greater than 2F+1 of the parties is required to reconstruct the key after sharing,
and use the DAG to reveal shares after a transaction \fino{tx} ordering becomes committed.


% -----
\autoref{sec:sharereveal} below explores detailed mechanisms for implementing these functionalities. 

%reveal their individual shares of the transaction key \fino{tx-key} and 


The key insight for operating \OTR on a DAG is that
each view must wait until \fino{Reconstruct(tx)} succeeds on transactions \fino{tx} of the previous view. 
In this way, a each view has dual purpose. 
First,
it commits blindly a new batch of transactions to the total ordering.
Second, 
it causally follows enough shares to open all previously committed transactions,
setting a deterministic opening.

The next section describes the
\fino{Protect-Reveal-Reconstruct} mechanism. 
Afterwards, we put everything together into a protocol in \autoref{sec:fino}.



==> sec/pcode.tex <==
\begin{algorithm}[b!]
    \small
    \caption{Fino's main event-handling loop. We omit validation and basic sanity checks on DAG \fino{deliver()} events.}
	\label{alg:fino}
    \SetKwProg{func}{function}{}{}

    \func{on deliver(vote(r))}{
        DAG[r].votes.add(vote)\;
        \If{|DAG[r].votes|>F}{
            commit(DAG[r].proposal) into DAG.allCommitted\;
            \For{tx $\in$ DAG.allCommitted}{
                \If{tx.myShare $\not\in$ tx.shares}{
                    broadcast(Reveal(tx) -- {\em optimistic})\;
                }
                \If{|tx.shares|>2F $\wedge$ Reconstruct(tx.shares) fails}{
                    broadcast(Reveal(tx) -- {\em pessimistic})\;
		}
            }
            \For{tx $\in$ DAG[r].encrypted}{
                \If{|tx.shares|>2F}{
                Reconstruct(tx)\;
                }
            }
        }
        checkViewChange()\;
    }

    \func{on deliver(share)}{
        tx $\leftarrow$ DAG.txs[share.txID]\;
        tx.shares.add(share)\;
        checkViewChange()\;
    }

    \func{on deliver(complaint(r))}{
        DAG[r].complaints.add(complaint)\;
        checkViewChange()\;
    }

    \func{on CommitTimeout()}{
         broadcast(complaint(r))\;
     }

    \func{checkViewChange()}{
        viewA$\leftarrow$ |DAG[r].votes| > F $\vee$ |DAG[r].complaints| > 2F\;
        viewB$\leftarrow$ True\;
        \For{tx $\in$ DAG.allCommitted}{
            \If{|tx.shares| < 2F + 1 $\vee$ Reconstruct(tx.shares) fails}{
                viewB$\leftarrow$False\;
                break\;
            }
        }
        \If{viewA and viewB}{
            r $\leftarrow$ r+1\;
            \If{self == DAG[r].leader}{
                broadcast(proposal(r))\;
            }
        }
    }

\end{algorithm}



